Measurement of charm production at central rapidity in proton-proton collisions at $\sqrt{s} = 7$ TeV

The $p_{\rm T}$-differential inclusive production cross sections of the prompt charmed mesons $D^0$, $D^+$, and $D^{*+}$ in the rapidity range |y|<0.5 were measured in proton-proton collisions at $\sqrt{s} = 7$ TeV at the LHC using the ALICE detector. Reconstructing the decays $D^0\rightarrow K^-\pi^+$, $D^+\rightarrow K^-\pi^+\pi^+$, $D^{*+}\rightarrow D^0\pi^+$, and their charge conjugates, about 8,400 $D^0$, 2,900 $D^+$, and 2,600 $D^{*+}$ mesons with 1<$p_{\rm T}$<24 GeV/$c$ were counted, after selection cuts, in a data sample of 3.14x10$^8$ events collected with a minimum-bias trigger (integrated luminosity $L_{\rm int}$ = 5/nb). The results are described within uncertainties by predictions based on perturbative QCD.

==> decay2_dstar.tex <==
With the track selection described in the previous paragraph, the acceptance in rapidity for D mesons
drops for $|y|\gsim 0.5$ at low $\pt$ and $|y|\gsim 0.8$ for $\pt\gsim 5~\gev/c$. 
A sharp cut $|y|<y_{\rm acc}(\pt)$ was applied, with $y_{\rm acc}$ smoothly increasing from 0.5 to 0.8 in
$0<\pt<5~\gev/c$.
$\Dzero$, $\Dplus$, and $\Dstar$ candidates were filtered by applying kinematical and topological cuts,
and particle identification.
For $\Dzero$, the two decay tracks were required to have 
a transverse momentum larger than $0.7~\gev/c$ and a normalized impact parameter, $d_0/\sigma_{d_0}$,
larger than $0.5$.
%An upper cut $d_0<1~\mm$ was applied to reject pairs of
%secondary tracks coming from decays far from the primary vertex (mainly of 
%strange hadrons) or particle interactions in the material.
Secondary vertices were required to have a minimum displacement of $100~\mum$ from the primary vertex
and a maximum distance of closest approach between the two tracks of $300~\mum$.
The cut $|\cos\theta^*|<0.8$ on the rest-frame decay angle was applied to reduce 
the contamination of background candidates that do not represent real two-body decays and have 
typically large values of $|\cos\theta^*|$.
Well-displaced $\DtoKpi$ topologies are characterized by large and opposite-sign values
of the decay track impact parameters ($d_0^{\pi}$ and $d_0^{\rm K}$) and good pointing of the reconstructed 
$\Dzero$ momentum to the primary vertex, i.e. a small value of the pointing angle $\theta_{\rm pointing}$
between the momentum and flight line.
Due to the strong correlation of these two features in the signal, the request 
$d_0^{\pi}\times d_0^{\rm K}\lsim (120~\mum)^2~(c\tau)^2???$ and $\cos\theta_{\rm pointing}\gsim 0.8$
was found to be effective in increasing the signal-to-background ratio.
The actual selection was loosened with increasing momentum in order to optimize 
the statistical significance of the signal.

The $\Dplus$ selection strategy is based on a similar approach as for the $\Dzero$.
The cut on the $\pt$ of single tracks is applied at 0.4~GeV/$c$ due to the lower average
momentum of the daughters of a three-body decay.
The candidate triplets are selected on the basis of the sum of the distances of the
daughter tracks to the reconstructed decay vertex, the decay length, the cosine of the
pointing angle and the sum of the squares of the $r\varphi$ impact parameters 
of the three tracks.
The applied cut values are $\pt$ dependent and are optimized in order to maximize
the statistical significance.
In particular, the decay length cut ranges from 900 $\mum$ in the lowest $\pt$ bin
to 1.15 mm at high $\pt$, $\cos\theta_{\rm pointing}$ is required to be above 0.95
at low $\pt$ and above 0.93 at higher $\pt$ and the cut on
$\Sigma\,d^2_0$ varies from $280\,000~\mum^2$ at low $\pt$ and $88\,000~\mum^2$ 
at high $\pt$.

The $\Dstar$ candidates were filtered applying kinematical selections on the final decay products and cuts on the topology of the $\Dzero$ decay. The kaon and pion originated from the $\Dzero$ decay were required to have a minimum transverse momentum $\pt>0.4~\gev/c$ while the minimum transverse momentum of the soft pion was set to $0.06 ~\gev/c$.
The variables used to select the topology of the  $\Dzero$ decay are similar to the one used for the $\Dzero$ analysis and were already explained in this paper.
%However, since the resolution in the invariant mass difference $\Delta m = m_{\Dstar} - m_{\Dzero} $ is defined only by the momentum resolution of the soft pion, the $\Dstar$ signal is expected as a narrow peak in the $\Delta m$ distribution.
However, the signal once evaluated in the invariant mass difference $\Delta m$ is close to the phase space boundary and thus on a low combinatorial background region. This feature allows us to apply relaxed selections on the topology of the $\Dzero$ decay maximizing the $\Dstar$ yield with a relatively low increase in the combinatorial background and with an excellent signal to background ratio. Above $\Dstar ~\pt>6~\gev/c$ the cuts on the distance of closest approach, $K$ and $\pi$ impact parameters and their product are set close to the limit of the experimental distributions, allowing to keep almost 100$\%$ of the signal. At low transverse momentum, $\pt<3~\gev/c$, the background topology resemble the signal one and so tighter selections, close to the one used in the $\Dzero$ analysis, are applied. 


The particle identification selection used information from the TPC and TOF
detectors, i.e. specific energy deposit and time-of-flight, respectively. 
In order to assign the kaon and/or pion mass to the decay tracks,
compatibility cuts were applied, in units of resolution ($\sigma$, cfr. section~\ref{sec:detector}), 
on the difference between the measured and expected signals. 
For both TPC and TOF, a $3\,\sigma$ compatibility cut was used. 
Tracks without a TOF signal were considered as both kaon and pion.
%The PID information from TOF and TPC is combined
%in such a way that a given particle is identified/discarded 
%as a kaon[pion] if at least one between TOF and TPC identifies/discards it as a kaon[pion].
%In case of conflict the track remains unidentified. 
%Tracks with a TPC $\dEdx$ signal compatible within $2\,\sigma$ 
%with the kaon (pion) hypothesis were used only as kaon (pion) in the momentum range 
%$p<0.6~\gev/c$. In the range $0.6<p<0.8~\gev/c$, where the pion and kaon
%expectations become closer, a $1\,\sigma$ selection was adopted.
%In the whole momentum range, tracks with a measured energy loss differing more than $3~\sigma$
%from that expected for kaons[pions] are discarded as possible kaons[pions].
%In the remaining cases the particle is tagged as kaon[pion]-compatible.
Two-prong candidates were accepted (as $\rm D^{0}$, $\rm \overline{D}^{0}$, or both) or rejected,
according to the compatibility with the $\rm K^\mp\pi^\pm$ final state.
For $\Dzero$ candidates used in $\Dstar$ reconstruction, the compatibility with the proper final state, 
known on basis of the soft pion charge, was checked. 
In the case of the $\Dplus \to \rm K^- \pi^+ \pi^+$ decay, the particle with the opposite charge sign
with respect to the D meson is a kaon. Hence, all triplets were rejected 
for which the opposite sign track is not compatible 
with the kaon hypothesis or
at least one of the two same sign tracks is not compatible with the pion hypothesis.

The comparison of the invariant mass distributions obtained with and without particle identification
selection showed that this selection reduced by a factor 2--3 the combinatorial background 
in the low $\pt$ region, while preserving close to 100\% of the D meson signal.


\begin{figure}[!t]
  \begin{center}
  \includegraphics[width=0.85\textwidth]{figures/InvMassPlot.eps}
  \caption{Invariant mass distributions of $\Dzero$,$\Dplus$,$\Dstar$ candidates for $\pt>2~\gev/c$. 
    The signal and background yields, extracted with a fit to the distributions (continuous lines) 
    along with the signal-peak sigma and mean as described in the text, are reported. 
    The dashed lines represent the background function in the 
    signal region.
  }
  \label{fig:invmass}
  \end{center}
\end{figure}
\begin{itemize}
\item Invariant mass analysis
\end{itemize}
The raw signal yields are extracted, in each $\pt$ interval,
by a fit to the invariant mass distributions, as shown in
Fig.~\ref{fig:invmass} for the $\pt$-integrated case.
For $\Dzero$ and $\Dplus$,
the fitting function consists of a Gaussian term describing 
the signal and an exponential term for the background.
For both mesons, the mean of the Gaussian is compatible
with the expected mass~\cite{pdg} within errors. The standard deviation,
an estimate of the invarian mass resolution, is well reproduced in Monte Carlo
simulations. 
For $\Dstar$ the fitting function consists of a Gaussian term describing 
the signal and a power law term for the background with threshold at the mass of the pion. The mean of the Gaussian is compatible
with the expected mass~\cite{pdg} within errors. The standard deviation,
an estimate of the invarian mass resolution, is well reproduced in Monte Carlo. 

 % as obtained after the
%selection described {\it above}. 
%The fit is performed in two steps: first, 
%the side-bands of the invariant mass histogram, where no signal is present, 
%are fit with the chosen background function. 
%Then, the total fit is performed using the information about background obtained from the first step.
The raw yields obtained are reported in Table...

